Tree Containment Above Minimum Degree is FPT

According to the classic Chv{\'{a}}tal's Lemma from 1977, a graph of minimum degree $\delta(G)$ contains every tree on $\delta(G)+1$ vertices. Our main result is the following algorithmic "extension" of Chv\'{a}tal's Lemma: For any $n$-vertex graph $G$, integer $k$, and a tree $T$ on at most $\delta(G)+k$ vertices, deciding whether $G$ contains a subgraph isomorphic to $T$, can be done in time $f(k)\cdot n^{\mathcal{O}(1)}$ for some function $f$ of $k$ only. The proof of our main result is based on an interplay between extremal graph theory and parameterized algorithms.

==> parts/stability-high-leaf-degree.tex <==
\section{Stability theorem for large leaf-degree}

We have showed that for $\ld(T)<k$, $\delta(G)>k^{\Omega(1)}$, $G$ always contains $T$ unless $G$ contains no $k^{\Omega(1)}$-escape vertices \emph{and} $T$ is \separable{$k^{\Omega(1)}$}.
The $\ld(T)<k$ constraint is very restrictive and narrows the class of trees the result is applicable to.

\begin{theorem}
	For every connected graph $G$ and a tree $T$ such that $|V(T)|=\delta(G)+k$ for $k>0$ and $\delta(G)\ge k^{\Omega(1)}$, one of the following holds:
	\begin{itemize}
		\item $G$ contains $T$ as a subgraph, or
		\item $G$ contains no $k^{\Omega(1)}$-escape vertices and $T$ is \separable{$k^{\Omega(1)}$}.
	\end{itemize}
\end{theorem}

Throughout the section, we assume that $|V(T)|=\delta(G)+k$ for $k>0$, $\delta(G)=k^{\Omega(1)}$, and $\ld(T)\ge k$.
\Cref{lemma:2k_path} allows us to only consider the case $\diam(T)<6k$.

